Statistical Physics of Deep Neural Networks: Generalization Capability, Beyond the Infinite Width, and Feature Learning

Deep Neural Networks (DNNs) excel at many tasks, often rivaling or surpassing human performance. Yet their internal processes remain elusive, frequently described as "black boxes." While performance can be refined experimentally, achieving a fundamental grasp of their inner workings is still a challenge. Statistical Mechanics has long tackled computational problems, and this thesis applies physics-based insights to understand DNNs via three complementary approaches. First, by averaging over data, we derive an asymptotic bound on generalization that depends solely on the size of the last layer, rather than on the total number of parameters -- revealing how deep architectures process information differently across layers. Second, adopting a data-dependent viewpoint, we explore a finite-width thermodynamic limit beyond the infinite-width regime. This leads to: (i) a closed-form expression for the generalization error in a finite-width one-hidden-layer network (regression task); (ii) an approximate partition function for deeper architectures; and (iii) a link between deep networks in this thermodynamic limit and Student's t-processes. Finally, from a task-explicit perspective, we present a preliminary analysis of how DNNs interact with a controlled dataset, investigating whether they truly internalize its structure -- collapsing to the teacher -- or merely memorize it. By understanding when a network must learn data structure rather than just memorize, it sheds light on fostering meaningful internal representations. In essence, this thesis leverages the synergy between Statistical Physics and Machine Learning to illuminate the inner behavior of DNNs.

==> src/acknowledgments.tex <==

\begin{multicols}{2}
    


Cari stimati lettori,\\
\vspace*{8mm}    


Se siete arrivati fin qui, o se siete saltati fin qui, probabilmente sperate di trovare il vostro nome in questa lista. Beh, è molto probabile che, se siete arrivati fin qui, lo troverete.

Permettetemi di iniziare con una nota di sublime gratitudine rivolta al mio stimatissimo supervisor, il Prof. Francesco Ginelli. Egli ha saputo trasformare quello che sarebbe potuto essere un periodo di studi severo e monotono in un'esperienza colma di insegnamenti preziosi e rallegrata da momenti di risate e felicità. Mai avrei immaginato che un dottorato potesse essere tanto piacevole, e questo, senza dubbio, grazie alla sua guida illuminata e alla sua ineguagliabile saggezza.

Procedendo, devo estendere i miei più sentiti ringraziamenti al Dr. Pietro Rotondo, il mio esimio cosupervisore. Egli mi ha sempre accolto nei suoi affascinanti progetti di ricerca con un'infinita generosità di spirito e di conoscenza. Pensate, miei cari, che peccato sarebbe stato, col senno di poi, se avessi optato per seguirlo sulla Barceloneta!

Non posso non menzionare la gentile e sempre disponibile Dr. Rosalba Pacelli. Sebbene i nostri punti di vista possano talvolta divergere, il suo costante supporto e la sua inestimabile assistenza sono stati per me di grande valore.

Un ulteriore tributo accademico è d'obbligo per il Prof. Marco Gherardi. A lui devo la mia gratitudine per aver pazientemente ascoltato le mie idee, a volte stravaganti, e per averle sapientemente guidate verso una direzione più appropriata.

Ma ora, volgiamo lo sguardo al di fuori delle austere mura dell'accademia e rivolgiamoci al mondo esterno, dove ho trovato rifugio tra amici leali e devoti. Ai miei compagni di ufficio va il mio più sentito ringraziamento per avermi regalato momenti di relax e divertimento, fondamentali per affrontare con serenità le sfide del lavoro. Un ringraziamento speciale va al Dr. Giuseppe Fava e al Dr. Martino Brambati, i cui contributi alla quantità e qualità dello svago sono stati ineguagliabili. Ora che questo viaggio è giunto al termine, mi chiedo, a chi attribuirete la colpa della vostra eterna ricreazione?

Continuando sul tema dello svago, il mio caro \textit{ton} milanese merita una menzione speciale. Giocare, ridere e scherzare con voi è stato un piacere incommensurabile, nonostante le mie continue ammonizioni domenicali riguardo al destino delle vostre mani, che spesso meriterebbero un luogo più oscuro.

Ritornando con affetto ai ricordi d'infanzia, vorrei esprimere la mia profonda gratitudine ai miei amici di lunga data. Sebbene la distanza ci separi, vi porto sempre nel cuore, nei gesti e nelle speranze. Vi ringrazio dal profondo del cuore, ben conscio del fatto che se son così, è sia colpa che merito vostro.

Permettetemi ora di rischiare la banalità agli occhi di chi mi conosce bene, ma i miei amici dell'università meritano un ringraziamento speciale. I Dr. Matteo Cagiada, Guglielmo Canziani, Ilaria Cucchetti e Stefano Callegaro sono stati per me come diamanti preziosi: cercati a lungo tra molte pietre, e una volta trovati, mai lasciati andare.

Volgendo ora lo sguardo alla mia famiglia, inizio con un ringraziamento affettuoso alla mia cara nonna RosaEmilia Bianchi. Grazie, cara nonna, per aver sempre preteso il meglio da me, anche attraverso le tue amorevoli, seppur vigorose, dimostrazioni d'affetto. Le tue carezze, se così possiamo definirle, sono state per me una costante fonte di ispirazione e motivazione.

Proseguendo, desidero ringraziare la mia adorata famiglia tutta. Spero di avervi dato almeno la metà di quello che voi avete generosamente dato a me.

Una menzione speciale va alla Dr. Chiara Ariosto, membro eminente della mia famiglia, che ha giocato un ruolo cruciale, anche solo aiutandomi a creare la mia password. Cara Chiara, le tue capacità sono state per me un faro di luce in un mare di codici e simboli.

Un ringraziamento altrettanto sentito va alla mia incantevole compagna, la Ms. Prashadini S. Kuruppu A.D. Sebbene la nostra strada non sia sempre stata priva di ostacoli, è stato un onore e un piacere incommensurabile condividere questi anni con te. Con la speranza che ne seguano molti altri, ti ringrazio dal profondo del cuore per avermi sempre donato il meglio di te stessa e per aver reso il sottoscritto una persona migliore, sotto ogni punto di vista.

Infine, ma non per importanza, vorrei esprimere la mia eterna gratitudine ai miei genitori. Se devo essere sincero, raramente ho trovato le parole giuste per ringraziarvi come meritate. Tuttavia, senza il vostro incondizionato supporto, nulla di tutto ciò sarebbe stato possibile. Permettetemi quindi, per una volta, di farlo per bene. Grazie, cari genitori, per avermi sempre supportato, anche quando le cose non andavano per il verso giusto. Grazie per avermi sempre spronato a fare di più e a fare meglio. Grazie per avermi sempre dato la possibilità di scegliere e di sbagliare. Grazie per avermi sempre fatto sentire amato.

Siamo giunti alla fine di questa lista, e forse vi starete chiedendo dov'è il vostro nome. Beh, se non lo avete trovato, non disperate. Potrebbe essere che non vi abbia ringraziato esplicitamente, ma non per questo non vi abbia apprezzato (anche solo per aver letto questa lista).

Infine, cari lettori, prima di lasciarvi permettetemi di fare un'ultima considerazione. Ai lettori meno esperti, potrebbe apparire che questa lista sia semplicemente un tributo a coloro che mi hanno sostenuto nel corso degli anni. Tuttavia, se avete letto con la dovuta attenzione e perspicacia, avrete compreso che questa lista è anche, e soprattutto, un omaggio a questo stesso Autore. Perché, miei cari, pur consapevole della mia mancanza di quella umiltà tanto celebrata e lodata in questo mondo in dirvi ciò, ho ``trionfato", ma non nel modo che penserete voi.

Nonostante le malelingue che predicevano che il mondo mi avrebbe schiacciato, che mi consideravano come l'attrezzo meno affilato del cassetto. Nonostante quei sempliciotti che con arroganza alzavano il pollice e l'indice sulla fronte in segno di scherno. Nonostante gli anni siano passati inesorabili e il tempo non si è mai fermato. Nonostante le innumerevoli occasioni in cui sono stato costretto a occupare il posto che gli altri avevano designato per me, adeguandomi a ruoli che non mi appartenevano.

Nonostante tutto ciò, o grazie a tutto ciò, miei affezionati lettori, ho compreso una verità fondamentale: vivere senza divertirsi è vivere a metà. %La gioia, il piacere, il divertimento sono l'essenza stessa della vita. 
Ho capito che perdendo il desiderio di essere il più brillante del branco, ho evitato la mediocrità che per altri è di per sé un trionfo. Perché, in fondo, questo vasto mondo è pieno di meraviglie da esplorare e di esperienze da vivere, e non prendere la strada panoramica sarebbe stato un errore imperdonabile. Se non avessi avuto il coraggio di esplorare ogni possibilità, di seguire ogni sentiero, non avrei mai scoperto il vero significato del viaggio.

E ora, miei cari, se non tentassi di risplendere con tutta la mia forza, come potrei mai aspirare a brillare un giorno? %Come potrebbe lo spirito umano gioire se non affrontato ogni sfida con un sorriso sulle labbra e una scintilla di speranza nel cuore?

Con queste parole, tali da far spaccare la bocca, miei cari lettori, vi lascio per sempre. O almeno, fino alla prossima lista di ringraziamenti.\\
\vspace*{8 mm}

\begin{flushright}
Sinceramente vostro,\\
Mr. Sebastiano Ariosto\\
\end{flushright}

\end{multicols}

\newpage


\begin{multicols}{2}
    
    Dear esteemed readers,\\
    \vspace*{8mm}    
    
    If you have made it this far, or if you have skipped ahead to this point, you are probably hoping to find your name on this list. Well, it is very likely that if you have come this far, you will find it.
    
    Allow me to begin with a note of sublime gratitude directed at my esteemed supervisor, Prof. Francesco Ginelli. He has managed to transform what could have been a period of severe and monotonous studies into an experience filled with valuable lessons, laughter, and happiness. Never could I have imagined that a PhD could be so pleasant, and this is undoubtedly thanks to his enlightened guidance and unparalleled wisdom.
    
    Proceeding, I must extend my most heartfelt thanks to Dr. Pietro Rotondo, my esteemed co-supervisor. He has always welcomed me into his fascinating research projects with infinite generosity of spirit and knowledge. Imagine, my dear readers, what a pity it would have been, in hindsight, if I had opted to follow him to Barceloneta!
    
    I must not fail to mention the kind and ever-available Dr. Rosalba Pacelli. Although our points of view may sometimes diverge, her constant support and invaluable assistance have been of great value to me.
    
    A further academic tribute is due to Prof. Marco Gherardi. To him, I owe my gratitude for patiently listening to my sometimes extravagant ideas and for wisely guiding them towards a more appropriate direction.
    
    But now, let us turn our gaze beyond the austere walls of academia and look to the outside world, where I have found refuge among loyal and devoted friends. To my office mates, I extend my heartfelt thanks for providing me with moments of relaxation and amusement, essential for facing work challenges with serenity. A special thanks goes to Dr. Giuseppe Fava and Dr. Martino Brambati, whose contributions to the quantity and quality of our leisure time have been unparalleled. Now that this journey has come to an end, I wonder, whom will you blame for your perpetual recreation?
    
    Continuing on the theme of leisure, my dear Milanese \textit{ton} deserves a special mention. Playing, laughing, and joking with you has been an immeasurable pleasure, despite my continual Sunday admonitions regarding the fate of your hands, which often deserve a darker place.
    
    Returning fondly to childhood memories, I would like to express my profound gratitude to my lifelong friends. Although distance separates us, I carry you always in my heart, in my gestures, and in my hopes. I thank you from the bottom of my heart, fully aware that if I am the way I am, it is both your fault and your merit.
    
    Allow me now to risk seeming banal to those who know me well, but my university friends deserve a special thanks. Dr. Matteo Cagiada, Guglielmo Canziani, Ilaria Cucchetti, and Stefano Callegaro have been like precious diamonds to me: sought for a long time among many stones, and once found, never let go.
    
    Turning now to my family, I begin with a heartfelt thank you to my dear grandmother RosaEmilia Bianchi. Thank you, dear grandmother, for always demanding the best from me, even through your loving, albeit vigorous, displays of affection. Your caresses, if we can call them that, have been a constant source of inspiration and motivation for me.
    
    Continuing, I wish to thank my beloved entire family. I hope I have given you at least half of what you have generously given to me.
    
    A special mention goes to Dr. Chiara Ariosto, an eminent member of my family, who played a crucial role, even just by helping me create my password. Dear Chiara, your skills have been a beacon of light in a sea of codes and symbols for me.
    
    An equally heartfelt thanks goes to my enchanting partner, Ms. Prashadini S. Kuruppu A.D. Although our path has not always been free of obstacles, it has been an immeasurable honor and pleasure to share these years with you. With the hope that many more will follow, I thank you from the bottom of my heart for always giving me your best and for making me a better person in every way.
    
    Finally, but not least, I would like to express my eternal gratitude to my parents. If I must be honest, I have rarely found the right words to thank you as you deserve. However, without your unconditional support, none of this would have been possible. So please allow me, for once, to do it properly. Thank you, dear parents, for always supporting me, even when things were not going well. Thank you for always encouraging me to do more and do better. Thank you for always giving me the opportunity to choose and to make mistakes. Thank you for always making me feel loved.
    
    We have reached the end of this list, and you may be wondering where your name is. Well, if you have not found it, do not despair. It may be that I have not explicitly thanked you, but that does not mean I have not appreciated you (even just for reading this list).
    
    Finally, dear readers, before I leave you, allow me to make one last consideration. To the less experienced readers, it may appear that this list is simply a tribute to those who have supported me over the years. However, if you have read with due attention and insight, you will have understood that this list is also, and above all, a homage to the Author himself. Because, my dear readers, although I am aware of my lack of that humility so celebrated and praised in this world in telling you this, I have ``triumphed", but not in the way you might think.
    
    Despite the naysayers who predicted the world would roll me, who considered me not the sharpest tool in the shed. Despite those simpletons who arrogantly raised their thumb and index finger to their foreheads in mockery. Despite the years passing inexorably and time never standing still. Despite the countless occasions when I was forced to be fed to others' rules and I even hit the ground running for that.
    
    Despite all this, or thanks to all this, my dear readers, I have understood a fundamental truth: didn't make sense not to live for fun. I have realized that by losing the desire to be the most brilliant of the pack, I avoided the head-dumb that for others is itself a triumph. Because, in the end, there is so much to see and so much to do in this world, that not taking the back street would have been an unforgivable mistake. If I had not had the courage to explore every possibility, to follow every path, I would never have discovered the true meaning of the journey.
    
    And now, my dear readers, if I did not try to glow with all my might, how could I ever aspire to shine one day?
    
    With these Mouth-Smashing words, dear readers, I leave you forever. Or at least, until the next list of acknowledgements.\\
    \vspace*{8 mm}
    
    \begin{flushright}
    Sincerely yours,\\
    Mr. Sebastiano Ariosto\\
    \end{flushright}
    
    \end{multicols}

==> src/titlepage.tex <==
\begin{titlepage}
	\newcommand{\HRule}{\rule{\linewidth}{0.5mm}}
	
	\center
	
    {
        \includegraphics[width=0.2\textwidth]{img/logo.jpg}\\[0.5cm] 
        \textsc{\Large Università degli Studi di Milano}\\[0.25cm]
        \textsc{\large Department of Physics}\\[0.5cm]
        \textsc{PhD School in Physics, Astrophysics, and Applied Physics}\\[0.25cm]
	    \textsc{XXXIV cycle}
    }

    \vfill
    \vfill
	
    {
        \HRule\\[0.4cm]
        \textsc{\Large\bfseries
            Data structure in machine learning
        }\\[0.1cm]
        \HRule
    }

    \vfill

    \begin{center}
        \large
        \textsc{Doctoral thesis of Vittorio Erba}\\ % Your name
    \end{center}

    \vfill

    \begin{minipage}[t]{0.4\textwidth}
        \large
        \textsc{\small School director}\\
        Matteo \textsc{Paris}

        \vspace{1cm}
        \textsc{\small Referees}\\
        {\color{red}COMPLETE}\\
        {\color{red}COMPLETE}
    \end{minipage}
    \begin{minipage}[t]{0.4\textwidth}
        \flushright
        \large
        \textsc{\small Supervisor of the thesis}\\
        Sergio \textsc{Caracciolo}

        \vspace{1cm}
        \textsc{\small Evaluating commission}\\
        {\color{red}COMPLETE}\\
        {\color{red}COMPLETE}\\
        {\color{red}COMPLETE}
    \end{minipage}

    \vfill
    \vfill
	
    {
	    \textsc{Academic year 2020-2021}
    }
	
	\vfill
	
\end{titlepage}

%----------------------------------------------------------------------------------------


